Closeness Centrality Algorithms For Multilayer Networks

Centrality measures for simple graphs are well-defined and several main-memory algorithms exist for each. Simple graphs are not adequate for modeling complex data sets with multiple entities and relationships. Multilayer networks (MLNs) have been shown to be better suited, but there are very few algorithms for centrality computation directly on MLNs. They are converted (aggregated or collapsed) to simple graphs using Boolean AND or OR operators to compute centrality, which is not only inefficient but incurs a loss of structure and semantics. In this paper, we propose algorithms that compute closeness centrality on an MLN directly using a novel decoupling-based approach. Individual results of layers (or simple graphs) of an MLN are used and a composition function developed to compute the centrality for the MLN. The challenge is to do this accurately and efficiently. However, since these algorithms do not have complete information of the MLN, computing a global measure such as closeness centrality is a challenge. Hence, these algorithms rely on heuristics derived from intuition. The advantage is that this approach lends itself to parallelism and is more efficient compared to the traditional approach. We present two heuristics for composition and experimentally validate accuracy and efficiency on a large number of synthetic and real-world graphs with diverse characteristics.

==> texFiles/Abstract.tex <==
Centrality measures for simple graphs are well-defined and several main-memory algorithms exist for each. Simple graphs are not adequate for modeling complex data sets with multiple - entities and relationships. Multilayer networks (MLNs) have been shown to be better suited, but there are very few algorithms for centrality computation \textit{directly} on MLNs. Typically, they are converted (aggregated or collapsed) to simple graphs using Boolean AND or OR operators to compute centrality, which is not only inefficient, but incurs loss of structure and semantics.

%% AR 06/01/2023: changed some lines in the paragraph from 1st to 3rd person
% In this paper, we propose algorithms that compute closeness centrality on a MLN \textit{directly} using a novel decoupling-based approach. Individual results of layers (or simple graphs) of a MLN are used and a composition function is developed to compute the centrality for the MLN. The challenge is to do this efficiently preserving accuracy of results. However, since these algorithms do not have complete information of the MLN, computing a global measure such as closeness centrality is a challenge. Hence, these algorithms rely on heuristics derived from intuition. The advantage is that this approach lends itself to parallelism and is more efficient compared to the traditional approach. We present two heuristics for composition and empirically validate -- accuracy and efficiency -- on a large number of synthetic and real-world graphs with diverse characteristics. 
In this paper, algorithms have been proposed that compute closeness centrality on a MLN \textit{directly} using a novel decoupling-based approach. Individual results of layers (or simple graphs) of a MLN are used and a composition function is developed to compute the centrality for the MLN. The challenge is to do this efficiently preserving accuracy of results. However, since these algorithms do not have complete information of the MLN, computing a global measure such as closeness centrality is a challenge. Hence, these algorithms rely on heuristics derived from intuition. The advantage is that this approach lends itself to parallelism and is more efficient compared to the traditional approach. Two heuristics have been presented for composition and their accuracy and efficiency have been validated on a large number of synthetic and real-world graphs with diverse characteristics. 

\begin{comment}

\begin{abstract}
\setlength{\parindent}{5ex}
Centrality measures for simple graphs are well-defined and several main-memory algorithms exist for each. Simple graphs are not adequate for modeling complex data sets with multiple - entities and relationships. Multilayer networks (MLNs) have been shown to be better suited, but there are very few algorithms for centrality computation \textit{directly} on MLNs. They are converted (aggregated or collapsed) to simple graphs using Boolean AND or OR operators to compute centrality, which is not only inefficient, but incurs loss of structure and semantics.

%%As analysis of complex data not only uses graphs (connected or disconnected), but also multilayer networks (or MLNs) as it has a number of advantages from modeling and clarity perspective. Briefly, MLNs are layers where each layer is a graph and further nodes in two different layers could be same, but capture different relationships. This kind of MLNs where layers contain the same set of nodes are termed homogeneous MLNs (or HoMLNs) and are considered in this paper. Hence, it is relevant that we be able to compute centrality measures directly on MLNs.

%%Currently, HoMLNs are converted into a single graph using Boolean operations such as AND and OR and centrality measures are computed. This can serve as ground truth for direct computation of these measures. 
In this paper, we propose algorithms that compute closeness centrality on a MLN \textit{directly} using a novel decoupling-based approach. Individual results of layers (or simple graphs) of a MLN are used and a composition function developed to compute the centrality for the MLN. The challenge is to do this accurately and efficiently. However, since these algorithms do not have complete information of the MLN, computing a global measure such as closeness centrality is a challenge. Hence, these algorithms rely on heuristics derived from intuition. The advantage is that this approach lends itself to parallelism and is more efficient compared to the traditional approach. We present two heuristics for composition and experimentally validate --  accuracy and efficiency -- on a large number of synthetic and real-world graphs with diverse characteristics. 
%%algorithms for the closeness centrality for Boolean AND compositions. The decoupling-based approach computes desired centrality measure on each layer independently (or in parallel) and the results are composed to produce the centrality value for the two layers. This binary operation can be applied to more than two layers by using the previous result.

%%For the closeness centrality measure, we propose two heuristics that improve the accuracy with respect to ground truth and typically uses more information gathered from each layer. We hypothesize that more information used from each layer leads to better accuracy, but takes more computation effort. We provide intuition behind the heuristics proposed and provide extensive experimental results to support improved accuracy across graph characteristics. Large synthetic data sets are used to control graph characteristics and large real-world data sets are used to validate the hypothesis and accuracy consistency. We have also shown that the decoupling approach is more efficient than computation of ground truth,
\end{abstract}

%the analysis capability using our approach for modeling and efficient computation using MLNs. 
\vspace{-25pt}
\keywords{Multilayer Networks  \and Heuristics-Based \and Closeness Centrality \and Decoupling Approach \and Accuracy and Efficiency.}
\end{comment}


==> texFiles/Appendices.tex <==
\section{Appendix}
\label{sec:appendix}
\appendix

%%\textbf{Algorithm for Closeness Centrality Heuristic 1}


%%\textbf{Algorithm for Closeness Centrality Heuristic 2}



==> texFiles/DegreeCentrality.tex <==
\section{Degree Centrality}
\label{sec:degree_centrality}

The total number of edges that are incident on a node in a graph or monoplex is its degree. Degree hubs are nodes in a network that have a degree larger than or equal to the network's average degree. While degree hubs are specified for a single graph, there are no algorithms for calculating degree hubs for OR composed HoMLNs. In \cite{abhishek_hubify} Santra et. al. proposed three algorithms to estimate degree hubs in AND composed multilayer networks. If the HoMLN is turned into a single graph by a Boolean operation such as OR, we can expand the notion of a hub from a single graph to HoMLNs. In this paper, we suggest various composition functions to maximize accuracy and efficiency while estimating degree hub in OR composed multilayer networks. The ground truth is used to evaluate the performance and accuracy of our suggested heuristics for detecting the degree hubs of a multilayer network.

The degree centrality of a vertex $u$ in a network is defined as $C_{D}(u) = \textit{Number of adjacent neighbors}$. This value is divided by the maximum number of edges a vertex can have to normalize it. The equation for normalized degree centrality is $C_{D}(v) =  \frac{degree(v)}{n-1}$. High centrality hubs or degree hubs are the vertices with normalized degree centrality values higher than the other vertices. 

Even though there are different variations of degree centrality such as the group degree centrality \cite{everett1999centrality}, time scale degree centrality \cite{uddin2011time}, and complex degree centrality \cite{kretschmer2007new}, in this paper, we only address the normalized degree centrality for Boolean OR composed undirected homogeneous multilayer networks. We propose five algorithms to identify high centrality degree hubs in Boolean OR composed MLNs. We test the accuracy and efficiency of our algorithm against the ground truth. With extensive experiments on datasets of varying characteristics, we show that our approaches perform better than the naive approach and are efficient compared to the ground truth. 

For degree centrality, the ground truth is calculated as follows:

i. First, all the layers of the network are aggregated into a single layer using the Boolean OR composition function.

ii. Degree centrality of the aggregated graphs is calculated and the hubs are identified.

We compare the hubs computed by our algorithms against ground truth for accuracy. We use Jaccard’s coefficient as the measure to compare the accuracy of our solutions with the ground truth. We also use precision and recall as evaluation metrics to compare the accuracy of our solutions.

We aim to design solutions using the network decouple approach so that our accuracy for degree centrality is better than the naive approach and the efficiency is better than the ground truth. The naive approach when estimating the degree hubs in OR composed layers is the union of the degree hubs of the layers. Even though our solution works for any arbitrary number of layers, most of our experiments are done on networks with two layers.  

\subsection{Degree Centrality Heuristic 1 (DC1)}





==> texFiles/Heuristics.tex <==
\section{Heuristics}
\label{sec:heuristics}

\textbf{Symbols used in the pseudocode:}
\begin{center}
\captionof{table}{List of notations used.}
    \begin{tabular}{|p{2.5cm}|p{5cm}|}
        \hline
         \textbf{Symbol} & \textbf{Description}  \\
         \hline
         $CH_{x}$ & Closeness hubs of layer X.  \\
         \hline
         $CH_{y}$ & Closeness hubs of layer Y.  \\
         \hline
         $deg_{x}$ & A dict containing the degrees of nodes of layer X. \\
         \hline
         $deg_{y}$ & A dict containing the degrees of nodes of layer Y. \\
         \hline
         $sumDist_{x}(u)$ & Sum of paths from node $u$ to every other nodes in layer X. \\
         \hline
         $sumDist_{y}(u)$ & Sum of paths from node $u$ to every other nodes in layer Y. \\
         \hline
         $NBD_{x}(u)$ & One-hop neighbours of node $u$ in layer X. \\
         \hline
         $DH_{x}$ & Degree hubs of layer X.\\
         \hline
         $DH_{y}$ & Degree hubs of layer Y.\\
         \hline
    \end{tabular}
\end{center}

\textbf{Closeness Centrality:}
The following heuristics are designed to estimate closeness centrality hubs in Boolean AND composed layers.

\textbf{Layerwise Closeness Hub's Neighbor based approach (CC1):}


\begin{algorithm}
\caption{Procedure for Heuristic CC1}
\begin{algorithmic}[1]
\For{$u \in deg_{x}$}
    \State $degDistRatio_{x} \gets sumDist_{x}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\For{$u \in deg_{y}$}
    \State $degDistRatio_{y} \gets sumDist_{y}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\State $avg_{x} \gets mean(degDistRatio_{x})$
\State $avg_{y} \gets mean(degDistRatio_{y})$
\State $avgDegDistRatio_{xANDy} \gets max(avg_{x}, avg_{y})$
\For{$u \in CH_{x}$}
    \State $candidateNBD_{x}(u) \gets \emptyset$
    \For{$v \in NBD_{x}(u)$}
    \If{$degDistRatio_{x}(u) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{x}(u) \gets candidateNBD_x{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{y}$}
    \State $candidateNBD_{Y}(u) \gets \emptyset$
    \For{$v \in NBD_{y}(u)$}
    \If{$degDistRatio_{y}(u) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{y}(u) \gets candidateNBD_y{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{x} \cap CH_{y}$}
    \If{$|candidateNBD_{x} \cap candidateNBD_{y}| > 1$}
        \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup (candidateNBD_{x} \cap candidateNBD_{y})$
    \EndIf{}
    \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup u$
\EndFor
\end{algorithmic}
\end{algorithm}


\textbf{Estimated Summation of Path Length Based Approach(CC2): }

\begin{algorithm}
\caption{Procedure for Heuristic CC2}
\begin{algorithmic}[1]
\For{$u \in X.nodes$}
    \State $estSumDist_{xANDy} \gets max(dist_{x}(u), dist_{y}(u))$
\EndFor


\end{algorithmic}
\end{algorithm}



==> texFiles/Organization.tex <==
\section{Motivation/Introduction}

\textbf{4 to 5 pages pages}

why aggregate measures are important and where centrality measures are useful
Intro indicating the need, current single graph algos, and lack of algorithms for MLNs

\section{Related Work}

\textbf{2 pages}

aggregate algorithms and especially centrality algos. how closeness centrality algos work n single graphs
indicate they are main memory algorithms and hence has limitations on the size of graphs that can be analyzed

lack of centrality algos for MLNs and why they are important. also, how they can overcome some of the limitations of the main memory algos.
each layer can be analyzed separately increasing the total size of the graphs being analyzed. Can provide an example of OR compsoition
which does not work using main memorty algos

\section{MLN and the Decoupling Approach}

\textbf{1 or 2 pages}

advantages of decoupling approach from scalability and efficiency viewpoint. what is the approach.
how it is applied

how it preserves structure and semantics for drill down which is difficult in Boolean composed approaches

\section{Challenges for MLN algorithms}

\textbf{1 page}

1, why AND or OR compositions are not good for MLNs. size, subset usage etc.

2. MLN provides natural partitioning and how can we make use of it. also parallelizable

3. accuracy. is it possible to get the same accuracy as ground truth? what are the tradeoffs (wrt to information used or carried over)

4. efficiency: tradeoff between efficiency and accuracy

\section {Degree Centrality Algorithm for OR Booelan composition}

\textbf{2.5 to 3 pages }

definition, ground truth, naive approach as base line

intuition behind the heuristics; INCLUDE whatever you have developed

\subsection{Experimental Results and Analysis}

expt results discussion (need to figure out what and how much to put)

\section {Closeness Centrality heuristics and algorithms}

\textbf{3 to 5 pages}

need for alternative heuristics. trade-off between information used in composition wrt to accuracy
motivation behind heuristics
Big O complexity of algorithms 

\subsection{Experimental Results and Analysis}

\subsection{role of graph characteristics on accuracy and efficiency}

\section{Dealing with Multiple Layers and Effect on accuracy}

\textbf{1 page}

effect on accuracy as we add more layers (is it additive or multiplicative?)
the issues for using different heuristics for subsequent compositions

\section{Conclusions}

what is the punch line? how is it validated

\textbf{ 1 page}

\section{References}

\textbf{max 1 to 2 pages}

\underline{\textbf{Total Pages: 22 }} 

==> texFiles/discussion.tex <==
\section{Discussion on Accuracy vs. Efficiency}
\label{sec:discussion}




\begin{comment}


{\bf Lemma 1.1}
{\em If the communities in networks $G_x$ and $G_y$ are self-preserving, then the AND-combination of the communities produced by each of these networks will be same as the communities produced by the AND-composed network created from $G_x$ and $G_y$}
\begin{proof}
Consider two networks $G_x$ and $G_y$ that have the same set of vertices, but different set of edges. Moreover, both networks have only self-preserving communities. Now consider the network $G_{xANDy}$, which is the AND-composition of $G_x$ and $G_y$. Only edges that are in both $G_x$ and $G_y$ will be in the AND-composed network. Therefore the communities formed in the AND-composed network will be based on a subset of edges from $G_x$ and $G_y$. Since both $G_x$ and $G_y$ have self preserving communities, therefore the communities formed in $G_{xANDy}$ will be formed from the subsets of the communities in $G_x$ and $G_y$. Most importantly, due to the self preserving nature, no new grouping of vertices will be formed in $G_{xANDy}$. Therefore we can reconstruct the communities in $G_{xANDy}$ by taking the intersection of the communities of $G_x$ and $G_y$.
\end{proof}

\end{comment}
